SYMI: Efficient Mixture-of-Experts Training via Model and Optimizer State Decoupling

Mixture-of-Experts (MoE) models have become a widely-adopted solution to continue scaling model sizes without a corresponding linear increase in compute. During MoE model training, each input token is dynamically routed to a subset of experts -- sparsely-activated feed-forward networks -- within each transformer layer. The distribution of tokens assigned to each expert varies widely and rapidly over the course of training. To handle the wide load imbalance across experts, current systems are forced to either drop tokens assigned to popular experts, degrading convergence, or frequently rebalance resources allocated to each expert based on popularity, incurring high state migration overheads. To break this performance-accuracy tradeoff, we introduce SYMI, an adaptive MoE training system. The key insight of SYMI is to decouple the placement of expert parameters from their large optimizer state. SYMI statically partitions the optimizer of each expert across all training nodes. Meanwhile, SYMI dynamically adjusts the placement of expert parameters by repurposing existing weight updates, avoiding migration overheads. In doing so, SYMI right-sizes the GPU resources allocated to each expert, on a per-iteration basis, with minimal overhead. Compared to state-of-the-art MoE training systems, DeepSpeed and FlexMoE, SYMI is able to achieve a 30.5% and 25.9% faster time-to-convergence, respectively.

==> sections/figures/tex/model_drops.tex <==
%!TEX root =paper.tex
\begin{comment}
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{sections/figures/img/drop_quality2.pdf}
  \caption{TODO: X axis shows capacity factor. Two y axis. One showing latency, one showing number of tokens dropped.
  \myzhao{Just move this to be a table. Two rows for CF=1, CF=16.}
\askiad{Ok, so maybe drop the plot and pick 2/3 rows from the table below -- or I rerun it on 2 GPUs and iteration latency actually increases}}
  \label{fig:model_drops}
\end{figure}
\end{comment}

\begin{table}[t]
    \centering
    \caption{The percent of dropped tokens and normalized latency (lower is better) for GPT-125M with 32 experts across CF=1 and CF=16.}
    \label{tab:model_drops}
    \small
    \begin{tabular}{c c c}
        \hline
       \makecell{ \bf Capacity\\ \bf  Factor} & \makecell{ \bf Tokens\\ \bf  Drop \%} &   \bf Normalized Iteration Latency \\ \hline
        1               & 61.53       & 1.00              \\ \hline
        16              & 1.47        & 1.74          \\ \hline
    \end{tabular}
\end{table}

\begin{comment}

\begin{table}[h]
    \centering
    \caption{Label}
    \label{tab:performance_metrics}
    \small
    \begin{tabular}{c c c} % c}
        \hline
       \makecell{ \bf Capacity\\ \bf  Factor} & \makecell{ \bf Tokens\\ \bf  Drop \%} & \makecell{ \bf Average Iteration \\  \bf Latency (sec) } & \makecell{ \bf Loss After \\  \\ \hline \bf 1000 Iterations} \\ \hline
        1               & 61.53133       & 41.94022                   & 3.786544              \\ \hline
%        1.25            & 45.90802       & 41.60246                   & 3.603287              \\ \hline
%        1.5             & 37.76721       & 41.37571                   & 3.317450              \\ \hline
%        2               & 26.18684       & 39.72692                   & 2.797460             \\ \hline
        16              & 1.46575        & 72.85717                   & 1.285079              \\ \hline
    \end{tabular}
\end{table}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{sections/figures/img/motivation_capacity.png}
  \caption{TODO: will fix log scales, legends, data that tensorboard cut out (e.g. blue line\\
  TODO: add iteration time (higher for high capacity factors and \% of dropped tokens
  High capacity factor allows for faster convergence}
  \label{fig:model_drops}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{sections/figures/img/motivatino_moe_loss.png}
  \caption{
  How moe laod-balancing loss (mlc) works. Adding a factor to laod-balance the expert selection. The highest the mlc coefficient, the more you load balance}
  \label{fig:model_drops}
\end{figure}


\begin{figure}[t]
  \centering
  % \includegraphics[width=\linewidth]{example-image-golden} 
  \includegraphics[width=\linewidth]{sections/figures/img/motivation_mlc.png} 
  \caption{convergence for different moe load-balancing differential cost (mlc). \\
  x-axis: samples (2K tokens per sample), y-axis loss (low is good) \\
  No load balancing is bad, experts starve and it's like we don't have them. For mlc > 0, the smaller the better for convergence. \\
  }
  \label{fig:model_drops}
\end{figure}

\end{comment}

==> sections/figures/tex/model_loss.tex <==
%!TEX root =paper.tex
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{sections/figures/img/capacity_train_loss.pdf}
  \caption{Loss curve when training GPT-125M with 32 experts, across increasing capacity factors.}
  \label{fig:model_loss}
\end{figure}


==> sections/figures/tex/offload.tex <==
%!TEX root =paper.tex
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{example-image-golden}
  \caption{Figure how expert paralellism in an MoE works, showing expert parallelism.alongside token routing/capacity.}
  \label{fig:offload}
\end{figure}

